Modeling Information Change in Science Communication with Semantically Matched Paraphrases

Whether the media faithfully communicate scientific information has long been a core issue to the science community. Automatically identifying paraphrased scientific findings could enable large-scale tracking and analysis of information changes in the science communication process, but this requires systems to understand the similarity between scientific information across multiple domains. To this end, we present the SCIENTIFIC PARAPHRASE AND INFORMATION CHANGE DATASET (SPICED), the first paraphrase dataset of scientific findings annotated for degree of information change. SPICED contains 6,000 scientific finding pairs extracted from news stories, social media discussions, and full texts of original papers. We demonstrate that SPICED poses a challenging task and that models trained on SPICED improve downstream performance on evidence retrieval for fact checking of real-world scientific claims. Finally, we show that models trained on SPICED can reveal large-scale trends in the degrees to which people and organizations faithfully communicate new scientific findings. Data, code, and pre-trained models are available at http://www.copenlu.com/publication/2022_emnlp_wright/.

==> tables/detection.tex <==

\begin{table}%[htp]
    %\setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.2}
    \centering
    \fontsize{10}{10}\selectfont
    \begin{tabular}{l c c c}
    \toprule %\thickhline
    Method & MSE & $\rho$ & $r_{s}$\\
    \midrule 
Paraphrase & $1.879_{0.000}$ & $0.371_{0.000}$ & $0.435_{0.000}$\\
NLI & $1.709_{0.000}$ & $0.445_{0.000}$ & $0.159_{0.000}$\\
\midrule
CiteBERT & $0.387_{0.025}$ & $0.860_{0.006}$ & $0.757_{0.004}$\\
MPNet & $0.410_{0.006}$ & $0.850_{0.002}$ & $0.759_{0.004}$\\
SciBERT & $0.392_{0.016}$ & $0.856_{0.005}$ & $0.760_{0.011}$\\
MiniLM & $0.411_{0.002}$ & $0.854_{0.001}$ & $0.780_{0.002}$\\
RoBERTa & $\mathbf{0.371_{0.018}}$ & $\mathbf{0.867_{0.007}}$ & $\mathbf{0.787_{0.007}}$\\

    \bottomrule % \thickhline

    \end{tabular}
    \caption{MSE, Pearson correlation ($\rho$) and Spearman correlation ($r_{s}$) on predicting the similarity of the scientific findings for different models. Results are averaged over 5 random seeds; standard deviation is given in the subscript. } %Results are reported as the average macro F1 over 5 random seeds.}
    \label{tab:baseline-findings-matching}
\end{table}


==> tables/detection_easy.tex <==

\begin{table}%[htp]
    %\setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.2}
    \centering
    \fontsize{10}{10}\selectfont
    \begin{tabular}{l c c c}
    \toprule %\thickhline
    Method & MSE & $\rho$ & $r_{s}$\\
    \midrule 
MPNet & $1.350_{0.000}$ & $0.804_{0.000}$ & $0.477_{0.000}$\\
Paraphrase & $0.743_{0.000}$ & $0.647_{0.000}$ & $0.399_{0.000}$\\
NLI & $0.655_{0.000}$ & $0.693_{0.000}$ & $0.309_{0.000}$\\
MiniLM & $1.035_{0.000}$ & $0.845_{0.000}$ & $0.477_{0.000}$\\
\midrule
CiteBERT & $0.154_{0.042}$ & $0.957_{0.008}$ & $0.477_{0.000}$\\
MPNet-FT & $0.301_{0.012}$ & $0.928_{0.002}$ & $\mathbf{0.479_{0.000}}$\\
Longformer & $\mathbf{0.140_{0.048}}$ & $\mathbf{0.974_{0.010}}$ & $0.477_{0.000}$\\
SciBERT & $0.153_{0.027}$ & $0.956_{0.002}$ & $0.477_{0.000}$\\
Longformer-CT & $0.183_{0.107}$ & $0.955_{0.018}$ & $0.477_{0.000}$\\
MiniLM-FT & $0.285_{0.005}$ & $0.936_{0.001}$ & $0.479_{0.000}$\\
RoBERTa & $0.144_{0.035}$ & $0.966_{0.004}$ & $0.477_{0.000}$\\

    \bottomrule % \thickhline

    \end{tabular}
    \caption{MSE, Pearson correlation ($\rho$) and Spearman correlation ($r_{s}$) on predicting the similarity of the scientific findings for different models. Results are averaged over 5 random seeds; standard deviation is given in the subscript.} %Results are reported as the average macro F1 over 5 random seeds.}
    \label{tab:baseline-findings-matching}
\end{table}


==> tables/detection_hard_BACKUP.tex <==

\begin{table*}%[htp]
    \setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.2}
    \centering
    \fontsize{10}{10}\selectfont
    \begin{tabular}{l c c c | c c c | c c c}
    \toprule %\thickhline
    & \multicolumn{3}{c}{All} & \multicolumn{3}{c}{News} & \multicolumn{3}{c}{Twitter} \\
     \midrule
    Method & MSE & $\rho$ & $r_{s}$ & MSE & $\rho$ & $r_{s}$ & MSE & $\rho$ & $r_{s}$\\
    \midrule 
NLI & $2.921_{0.000}$ & $35.71_{0.00}$ & $23.48_{0.00}$ & $2.786_{0.000}$ & $35.78_{0.00}$ & $22.46_{0.00}$ & $3.255_{0.000}$ & $34.76_{0.00}$ & $23.00_{0.00}$\\
Paraphrase & $3.170_{0.000}$ & $23.58_{0.00}$ & $43.03_{0.00}$ & $3.310_{0.000}$ & $19.24_{0.00}$ & $43.83_{0.00}$ & $2.824_{0.000}$ & $35.41_{0.00}$ & $38.31_{0.00}$\\
MPNet & $0.718_{0.000}$ & $72.59_{0.00}$ & $73.15_{0.00}$ & $0.713_{0.000}$ & $74.76_{0.00}$ & $75.51_{0.00}$ & $0.730_{0.000}$ & $62.06_{0.00}$ & $61.99_{0.00}$\\
MiniLM & $0.628_{0.000}$ & $73.98_{0.00}$ & $74.91_{0.00}$ & $0.646_{0.000}$ & $76.27_{0.00}$ & $77.15_{0.00}$ & $0.583_{0.000}$ & $64.61_{0.00}$ & $65.85_{0.00}$\\
\midrule
SciBERT & $0.574_{0.010}$ & $72.98_{0.85}$ & $72.93_{0.54}$ & $0.584_{0.008}$ & $74.47_{0.90}$ & $74.43_{0.68}$ & $0.548_{0.022}$ & $65.80_{0.41}$ & $63.96_{0.03}$\\
CiteBERT & $0.576_{0.012}$ & $73.04_{0.63}$ & $72.79_{0.59}$ & $0.586_{0.003}$ & $74.42_{0.55}$ & $74.23_{0.71}$ & $0.553_{0.038}$ & $66.04_{1.84}$ & $63.60_{2.25}$\\
RoBERTa & $0.588_{0.020}$ & $74.87_{0.55}$ & $74.99_{0.93}$ & $0.613_{0.021}$ & $75.95_{0.83}$ & $76.02_{1.20}$ & $0.528_{0.057}$ & $\mathbf{69.60_{0.75}}$ & $\mathbf{66.91_{0.79}}$\\
MPNet-FT & $\mathbf{0.487_{0.002}}$ & $\mathbf{76.48_{0.04}}$ & $\mathbf{76.41_{0.10}}$ & $0.474_{0.003}$ & $78.66_{0.06}$ & $77.85_{0.12}$ & $\mathbf{0.521_{0.002}}$ & $66.61_{0.22}$ & $66.35_{0.27}$\\
MiniLM-FT & $0.492_{0.001}$ & $75.86_{0.04}$ & $75.70_{0.03}$ & $\mathbf{0.464_{0.001}}$ & $\mathbf{78.68_{0.04}}$ & $\mathbf{78.37_{0.05}}$ & $0.560_{0.003}$ & $63.79_{0.06}$ & $63.30_{0.28}$\\


    \bottomrule % \thickhline

    \end{tabular}
    \caption{MSE, Pearson correlation ($\rho$) and Spearman correlation ($r_{s}$) on predicting the similarity of the scientific findings for different models. Results are averaged over 5 random seeds; standard deviation is given in the subscript.} %Results are reported as the average macro F1 over 5 random seeds.}
    \label{tab:baseline-findings-matching}
\end{table*}


==> tables/detection_hard_OLD.tex <==

\begin{table}%[htp]
    %\setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.2}
    \centering
    \fontsize{10}{10}\selectfont
    \begin{tabular}{l c c c}
    \toprule %\thickhline
    Method & MSE & $\rho$ & $r_{s}$\\
    \midrule 
MPNet & $1.064_{0.000}$ & $0.591_{0.000}$ & $0.591_{0.000}$\\
Paraphrase & $3.181_{0.000}$ & $0.157_{0.000}$ & $0.161_{0.000}$\\
NLI & $2.916_{0.000}$ & $0.293_{0.000}$ & $0.145_{0.000}$\\
MiniLM & $1.002_{0.000}$ & $0.598_{0.000}$ & $0.613_{0.000}$\\
\midrule
CiteBERT & $0.654_{0.027}$ & $\mathbf{0.672_{0.012}}$ & $\mathbf{0.665_{0.012}}$\\
MPNet-FT & $\mathbf{0.534_{0.007}}$ & $0.666_{0.005}$ & $0.660_{0.005}$\\
Longformer & $0.676_{0.051}$ & $0.658_{0.022}$ & $0.658_{0.020}$\\
SciBERT & $0.665_{0.042}$ & $0.663_{0.010}$ & $0.653_{0.011}$\\
Longformer-CT & $0.852_{0.357}$ & $0.603_{0.068}$ & $0.605_{0.062}$\\
MiniLM-FT & $0.555_{0.002}$ & $0.636_{0.001}$ & $0.622_{0.003}$\\
RoBERTa & $0.672_{0.099}$ & $0.646_{0.022}$ & $0.646_{0.019}$\\

    \bottomrule % \thickhline

    \end{tabular}
    \caption{MSE, Pearson correlation ($\rho$) and Spearman correlation ($r_{s}$) on predicting the similarity of the scientific findings for different models. Results are averaged over 5 random seeds; standard deviation is given in the subscript.} %Results are reported as the average macro F1 over 5 random seeds.}
    \label{tab:baseline-findings-matching}
\end{table}


==> tables/detection_none.tex <==

\begin{table}%[htp]
    %\setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.2}
    \centering
    \fontsize{10}{10}\selectfont
    \begin{tabular}{l c c c}
    \toprule %\thickhline
    Method & MSE & $\rho$ & $r_{s}$\\
    \midrule 
MPNet & $1.217_{0.000}$ & $0.792_{0.000}$ & $0.767_{0.000}$\\
Paraphrase & $1.879_{0.000}$ & $0.371_{0.000}$ & $0.435_{0.000}$\\
NLI & $1.709_{0.000}$ & $0.445_{0.000}$ & $0.159_{0.000}$\\
MiniLM & $1.020_{0.000}$ & $0.817_{0.000}$ & $\mathbf{0.802_{0.000}}$\\
\midrule
CiteBERT & $0.387_{0.025}$ & $0.860_{0.006}$ & $0.757_{0.004}$\\
MPNet-FT & $0.410_{0.006}$ & $0.850_{0.002}$ & $0.759_{0.004}$\\
Longformer & $0.389_{0.020}$ & $0.864_{0.010}$ & $0.791_{0.006}$\\
SciBERT & $0.392_{0.016}$ & $0.856_{0.005}$ & $0.760_{0.011}$\\
Longformer-CT & $0.487_{0.135}$ & $0.832_{0.036}$ & $0.761_{0.022}$\\
MiniLM-FT & $0.411_{0.002}$ & $0.854_{0.001}$ & $0.780_{0.002}$\\
RoBERTa & $\mathbf{0.371_{0.018}}$ & $\mathbf{0.867_{0.007}}$ & $0.787_{0.007}$\\

    \bottomrule % \thickhline

    \end{tabular}
    \caption{MSE, Pearson correlation ($\rho$) and Spearman correlation ($r_{s}$) on predicting the similarity of the scientific findings for different models. Results are averaged over 5 random seeds; standard deviation is given in the subscript.} %Results are reported as the average macro F1 over 5 random seeds.}
    \label{tab:baseline-findings-matching}
\end{table}


==> tables/generation.tex <==

\begin{table}%[htp]
    %\setlength{\tabcolsep}{1.5pt}
    \def\arraystretch{1.2}
    \centering
    \fontsize{10}{10}\selectfont
    \begin{tabular}{l c c c}
    \toprule %\thickhline
    Method & R-1 & R-2 & R-L \\
    \midrule %\hline
T5 & $0.265_{0.010}$ & $0.164_{0.009}$ & $0.231_{0.009}$\\
BART & $\mathbf{0.327_{0.003}}$ & $\mathbf{0.218_{0.002}}$ & $\mathbf{0.290_{0.003}}$\\

    \bottomrule % \thickhline

    \end{tabular}
    \caption{ROUGE scores for paraphrase generation from paper findings to news findings.} %Results are reported as the average macro F1 over 5 random seeds.}
    \label{tab:generation}
\end{table}

